TunnelScatter: Low Power Communication for Sensor Tags using Tunnel Diodes

Due to extremely low power consumption, backscatter has become the transmission mechanism of choice for battery-free devices that operate on harvested energy. However, a limitation of recent backscatter systems is that the communication range scales with the strength of the ambient carrier signal(ACS). This means that to achieve a long range, a backscatter tag needs to reflect a strong ACS, which in practice means that it needs to be close to an ACS emitter. We present TunnelScatter, a mechanism that overcomes this limitation. TunnelScatter uses a tunnel diode-based radio frequency oscillator to enable transmissions when there is no ACS, and the same oscillator as a reflection amplifier to support backscatter transmissions when the ACS is weak. Our results show that even without an ACS, TunnelScatter is able to transmit through several walls covering a distance of 18 meter while consuming a peak biasing power of 57 microwatts. Based on TunnelScatter, we design battery-free sensor tags, called TunnelTags, that can sense physical phenomena and transmit them using the TunnelScatter mechanism.

==> sections/design.tex <==
In this section, we first provide a high-level overview of our architecture. We describe in detail, the various components that make up the architecture. First, we describe the design of the universal light sensor. Next, we describe an ultra-low power mechanism that offload  readings from the light sensor to a powerful end-device. Finally, we discuss the powerful end-devices that receive and interpret the light sensing information.



\subsection{\system: System Overview}
The fundamental operation of \system is to identify an action that is performed over a visible light sensor under ambient light such as a particular hand gesture movement or a person walking past the sensor. We design a battery-free sensor that utilizes ultra-low power mechanisms to capture, digitize, and communicate light information wirelessly without the use of any energy-expensive computational block. Instead, our sensor delegates all of the processing operations to an end device that runs a classifier algorithm to identify a particular action that is performed over the sensor. The classifier identifies an action by matching it to its unique pattern or \emph{footprint} in the perceived light readings. This enables our envisioned application scenarios, as mentioned in section~\ref{appscenario}.\av{This section will need to be updated with information of polymorphic sensor}

%At a high level, \system identifies a particular action that is performed over a light sensor such as a hand movement or a person walking past the sensor by classifying the emerging unique pattern or \emph{footprint} in the perceived light readings. Our architecture supports battery-free sensors that we devise, which utilize ultra-low power mechanisms to digitize and communicate light information in the time domain without the use of any energy-expensive computational blocks. Instead, our sensors leverage ambient backscatter communication and delegate all of the energy-expensive processing operations to a powerful end-device that runs the classification algorithm. Further, we develop a mechanism that, for an individual sensor, maximizes bandwidth-efficiency by forwarding all of the digitized sensor readings in the time-domain, thus keeping the frequency fixed. 

We face several key challenges to realize \system. First, the power consumption of an ADC significantly increases with its resolution and sampling frequency which makes it increasingly difficult to power the sensor from harvested energy, particularly at lower light levels. Thus, we are forced to trade-off these two properties in order to mitigate the power consumption while maintaining a sufficiently high detection accuracy at the end device.

%Thus, we have to trade-off sensing resolution and sampling frequency while maintaining a sufficient detection accuracy of sensed actions.
%where we are able to accurately represent complex actions such as hand gestures using a sufficiently high resolution and sampling frequency while maintaining detection accuracy.

Second, to communicate light readings wirelessly while maintaining ultra-low power consumption and efficient spectrum usage is a non-trivial problem. Prior methods leverage ambient backscatter to communicate sensor readings at microwatts of power, but sacrifice in spectrum bandwidth (few \SI{}{\mega\hertz}) due to the usage of mechanisms that frequency multiplex a large set of raw sensor data~\cite{what}. 

%to communicate a digitized set of data while optimizing for spectrum-efficiency requires a specialized method of forwarding the data to the transmitting antenna.

Finally, \ldots 

%using a single low-cost light sensor such as a solar cell or a photodiode to detect a complex action such as a hand gesture is a non-trivial problem.

\system overcomes the first challenge by employing an ultra-low power digitization mechanism based on a network of thresholding circuits that we design. To allow for the sensor to operate on harvested energy and to support ultra-low power transmissions, we leverage backscatter of ambient BLE and LoRa signals. Further, we devise a mechanism that optimizes for bandwidth-efficiency by forwarding the digitized data in the time-domain to a single transmitting backscatter antenna. Thus, \system communicates streams of digitized sensor readings which are then received and processed by the end device to reveal the light information. We describe our design choices next.

%This procedure is done in several steps. First, a battery-free light sensor collects the light patterns, digitizes them, and


\subsection{Polymorphic Light Sensor}
\input{sections/vls}

\subsection{Using Ambient Wireless Signals for Communication}
\input{sections/ambwireless}



\subsection{Processing at a Powerful End-device}

==> sections/designs.tex <==
\label{marker}




==> sections/discussion.tex <==

\fakepar{Ambient signals}  In this paper, we show that tunnel diodes act like a reflection amplifier, and backscatter a weak carrier signal to achieve a high  range. We can also use ambient wireless signals instead of carrier signals. The range of state-of-the-art ambient backscatter systems~\cite{abc,wifibackscatter,hitchike,fmbackscatter} suffer in the presence of a weak signal and  limits the practical deployment. We believe Quantumscatter could significantly improve the range of these systems, and hence significantly increase the scenarios for ambient backscatter systems.

\fakepar{Tunnel Diodes} Tunnel diodes were widely used in electronic devices close to half a century back. However, they were replaced slowly over the years by other CMOS components, and at present, they can be difficult to procure as very few manufacturers produce them. In this paper, we use tunnel diodes that were manufactured in the 1960s, which we purchased from an antique radio electronic store. These devices are not expensive to make and are also very resilient. We believe the encouraging results that we demonstrate in this paper, make a strong argument for manufacturing these devices at large scale again. 

\fakepar{Polymorphic Processing}






==> sections/evalharvest.tex <==
In this section, we evaluate the ability of different parts of our architecture to operate under the constraints of the harvested power. 

\fakepar{Energy Harvesting Time}

\fakepar{Fusion sensor}

\fakepar{Overall sensor}

\fakepar{}



==> sections/evaluation.tex <==
\subsection{Power consumption}

\subsection{Communication range}

\subsection{Switching between different modes}

\subsection{Dynamics of changing light conditions}

\subsection{Light sensor performance}

\subsection{Operation on harvested energy}

\subsection{Improving reliability with SpreadScatter}
\input{sections/evaluation/spreadscatter.tex}


\fakepar{Setup}

% Todo: 
% Put the images side-by side. Reduce text. 
% First fix aspect ratio of the images :)
% Begining of comment

\fakepar{ULP Digitization} Evaluate the 4-bit Flash ADC in terms of power consumption. Perhaps also add an image of how the digitization looks when performing a shadow over the light sensor. How well does it work with overlapping shadows?


\fakepar{Reception of Serial Backscatter Data} 
\begin{itemize}
    \item The accuracy of receiving the backscattered signals. At the receiver, we need to accurately detect when the antenna starts backscattering and when it stops. By detecting the start and the end of the backscattering period we can infer the duration of the digitized signal which allows us to properly reconstruct the analog signal. Any error in the detected backscatter duration has a significant impact on the accuracy of identifying sensed events.
\end{itemize}



%How does the choice of receiver impact the detection accuracy? 

\begin{itemize}
    \item FM
    \item LoRa (\SI{868}{\MHz})
    \item \SI{2.4}{\GHz}
\end{itemize}

\fakepar{Communication Range}
We perform experiments in an indoor office environment and outdoors.
\begin{itemize}
    \item FM
    \item LoRa (\SI{868}{\MHz})
    \item Bluetooth? (\SI{2.4}{\GHz})
\end{itemize}

\fakepar{Power Consumption} We perform a preliminary experiment to evaluate the power consumption of a commercial micro-controller running a low power periodic ADC. We choose the MSP430FR5969~\cite{msp430} micro-controller for this purpose due to its design being targeted towards ultra-low-power~(ULP) applications. We evaluate the power consumption of the MSP430FR5969 micro-controller when running a 12-bit ADC periodically. We program the micro-controller to use a timer to set the sampling rate of the ADC by triggering it to start its conversion at a specified frequency. When the ADC is inactive, the micro-controller stays in low power mode while waiting for the timer trigger signal. To measure the sampling period of the ADC, we program the micro-controller to toggle a GPIO before and after the conversion period of the ADC, and we measure the toggling frequency using a logic analyzer. Next, we disconnect the micro-controller from the programmer and instead power it at the minimum voltage required to enable \SI{1}{\kilo\hertz} of ADC sampling frequency, which we found to be \SI{2.2}{\volt}. 
% 2.2 V was the minimum voltage I used to get the expected frequencies. Not sure if necessary to mention this?

To measure the power consumption, we place a \SI{1}{\kilo\ohm} shunt resistor in series between the voltage source and the micro-controller. Next, we connect a logic analyzer across this resistor and measure the voltage drop over it. The power consumption then follows by calculating the current flow via Ohm's law, 
and multiplying the resulting current by the operating voltage value (\SI{2.2}{\volt}). We measure the power consumption of the micro-controller at three different sampling frequencies that are representative of our target applications: \SI{200}{\hertz}, \SI{500}{\hertz}, and \SI{1}{\kilo\hertz}. We collect the samples for \SI{3}{\second} of operation each, and compute the Root Mean Square~(RMS) value to determine the average power consumption during this period of operation. Table~\ref{adc-power} Shows the power consumption of the micro-controller when operating at \SI{2.2}{\volt} for the three aforementioned frequencies.
% Metric in sampling period or in frequency? Xia Zhou used sampling period in her latest paper.
\begin{table}
\caption{Average power consumption (RMS) of the MSP430FR5969 when running an ADC on a \SI{2.2}{\V} external supply.}
%\vspace{-4mm}
\label{adc-power}
\begin{tabular}{|l|l|l|}
\hline
Sampling frequency & Power consumption \\ \hline
\SI{200}{\Hz} & \SI{385}{\micro\watt} \\ \hline
\SI{500}{\Hz} & \SI{559}{\micro\watt} \\ \hline
\SI{1}{\kHz} & \SI{687}{\micro\watt}  \\ \hline

%Analog backscatter~ (\SI{100}{\kilo\hertz} - \SI{1}{\mega\hertz}) & \SI{2.0}{\V}  & \SI{19.5}{\micro\watt} - \SI{120}{\micro\watt} \\ \hline
\end{tabular}
\vspace{-4mm}
\end{table}

\fakepar{Temporal Resolution}
How long does it take to sense, transmit, and detect shadows? Examples of Questions: Sensing rate (e.g. solar cell vs photodiode), communication rate (minimum time it takes to perform serial backscatter), latency of reception (how long does it take to receive and extract useful information from the entire communicated sequence of bits?). All combined will set a fundamental time constraint on the ability of our system to detect variations in light levels or shadows.

\fakepar{Battery-free Operation Conditions}
How will it work in ambient light conditions? Can the system harvest sufficient energy in low light? What's the minimum operating conditions?

\fakepar{Multiple Visible Light Markers}


==> sections/floormarkers.tex <==
%Detecting the presence or absence of people, proximity to a sensor or their precise location is a significant problem that has attracted the significant attention of the research community~\cite{}. This enables application scenarios such as helping conserve energy in a home by turning off appliances or heating in the absence of people or using the location information to enable indoor navigation. State-of-the-art systems often require  instrumenting ambient environment with complex devices such as an RFID reader, modify ambient lighting with beaconing circuits, or deploy other sophisticated sensors all of which significantly increase the cost and the complexity of the deployment. We imagine the light sensors in our architecture can be placed on the floor,  walls or the door to enable several such application scenarios. As an example, in the Figure~\ref{} we demonstrate a scenario where the light sensors are in the form of a rug at the entrance of the door. The sensor detects crossing and the direction of crossing by observing the changes in the ambient light level and communicates to a device in the home which controls the heating based on the occupancy. In another scenario, as we show in the Figure~\ref{}, the light sensors are placed on the floor and programmed with location information. As the light sensor detects the presence of the person nearby, it broadcasts location information which is received and processed by a smart-phone. The location information helps the user navigate in the indoor environment.


\begin{figure}[t]
    \includegraphics[width=0.5\textwidth]{images/passiveSwitch.pdf} 
    \caption{\textit{Passive Switch.}  }
    \label{fig:passiveSwitch}
\end{figure}

==> sections/introduction.tex <==
Light is an integral part of our lives, and together with its numerous components influences us in a variety of ways.  Light can be broadly divided based on wavelength into several components: ultraviolet, visible and infrared light.  The visible light helps us see and experience the physical world. On the other hand, ultraviolet and infrared light is invisible to human eye as their wavelength is outside the region visible to the human eye. However, the invisible nature makes them appealing to sensing or communication, as it can be used without causing inconvenience to the people around. Light also impacts our health in different ways, too much exposure to the infrared light can cause various forms of cancer, or exposure to blue visible light can disrupt the sleep rhythms.   Hence, due to various impact of light on our health, 

Hence, due to the impact of light on our health, and the various applications that it enables, sensing light and its various components is  important capability. %%% Talk about some way of polymorphism of light sensor, different spectrum etc %%%%%%






%Sensing systems are increasingly becoming an important part of our life. We use these systems to interact with devices in our homes, mobile devices, personal computers etc.  


%Past several years has seen a significant interest and efforts to develop mechanisms and techniques to enable sensing capabilities such as hand gesture recognition~\cite{li2017reconstructing}, human posture reconstruction~\cite{li2015human,li2016practical}, indoor localization~\cite{epsilon,kuo2014luxapose}, human vitals monitoring (breath, heartbeat)~\cite{} etc. These capabilities support novel application scenarios such as indoor navigation~\cite{epsilon}. While there has been a sustained effort that has resulted in numerous sensing systems over the past decade, at the present, a vast majority of state-of-the-art sensing systems are not ubiquitous.


 %vast majority of existing sensing systems are prohibitively expensive,  they are difficult to deploy and maintain, and can negatively impact the physical and the radio environment. There are several reasons for these shortcomings: \emph{First}, many sensing systems use changes in the property of radio frequency~(RF) signals for sensing. RF spectrum is a shared medium that is used by a large number of devices contending for access which causes the problem of the  increased cross technology interference~(CTI)~\cite{}. \emph{Second}, a large number of these systems are expensive to deploy especially when done at any reasonable scale 



%due to the use of expensive components and the architecture. As an example, commodity radio transceivers or computational units such as micro controllers or FPGAs even when purchased at a scale can individually cost a few USD.

%hese systems can be expensive to both deploy and maintain. They often use components such as commodity radio transceivers, complex algorithms for inferring sensing tasks, and usually have batteries on the sensor devices which needs to be often frequently replenished. All of these challenges negatively impact the prospects of ubiquitous and sustianable deployment of the sensing systems. 

%To overcome these challenges of RF based sensing systems, several recent systems leverage alternative sensing medium such as vibration, light or heat for sensing applications. Among these mediums, visible light is among the most promising to bring ubiquitous sensing capabilities.



\fakepar{Contributions} We make several contributions in this work

\begin{enumerate} 
\item We investigate the trade-off in sensing and temporal resolution for visible light sensing applications. 
\item We devise an ultra-low power mechanism that digitises and transmit light sensor readings without overhead of local processing and 
\item We introduce first visible light sensing architecture that combines RF backscatter with visible light sensing to achieve a peak power consumption of \SI{20}{\micro\watt}s which helps support battery-free operation.
\item The second item 
\item The third etc \ldots 
\end{enumerate}


Our work is most closely related to the architecture presented by Varshney et al.~\cite{}. 












 

==> sections/relatedwork.tex <==
\fakepar{Computational overhead on backscatter sensors} There have been prior attempts that investigate the overhead of local processing on energy harvesting sensor platforms. Zhang et al. demonstrate that performing local processing is significantly energy expensive as compared to backscatter communication, and advocate eliminating computational blocks and redesigning the network stack to support ultra-low power consumption~\cite{ekhonet}. Talla et al. build on the insight of Zhang et al. and eliminate computational block, and couple microphone directly to a backscatter transmitter to send audio signals at peak power consumption of a few \SI{}{\micro\watt}s. Their design transmits audio signal at the same frequency as the carrier signal which requires complex self-interference cancellation mechanism and significant processing using an SDR for the reception. Naderiparizi et al.~\cite{hdcamera} develop a technique called PWM backscatter that can transmit analog signals from image sensors while keeping the backscattered signal apart in frequency from the carrier signal reducing self-interference and improving the SNR of the backscattered signal.  The backscattered signal is then received using an SDR. All of these systems require a sophisticated and dedicated device to transmit the carrier signal and to receive the weak backscatter reflections which negatively impacts the prospects of ubiquitous deployment.  Our work without involving computational block can backscatter ambient signals such as LoRa or FM for transmitting light sensor readings which eliminates the need for a dedicated device to generate the carrier signal. Further, our work can leverage signal strength detection that is available on inexpensive radio transceivers~\cite{freqshift}.  A  vast number of deployed wireless devices such as WiFi routers, LoRa base stations, smartphones employ such transceivers. The use of already available infrastructure reduces the cost of reception to support our vision of sustainable visible light sensing.

\fakepar{Radio frequency sensing} Past decade has seen a significant effort to develop novel radio frequency sensing capabilities. We divide the state-of-the-art RF sensing systems to two categores: 


Adib et al. demonstrate ability to detect vital human signs such as breath rate or heart beat by tracking changes in the properties of RF signal~\cite{adibsmarthome}.

\fakepar{Backscatter communication}


\fakepar{Visible light sensing and communication} Due to the concerns like increased cross technology interference, privacy concerns etc, past several years has seen a significant interest to develop visible light as an alternative to RF for sensing and communication application. 

Existing visible light sensing systems can be broadly divided into two categories, in the first category we have systems that require instrumenting users or objects with an active device that receives visible light 
beacons which helps support applications such as localization. 






==> sections/scenariosandreq.tex <==


\input{sections/requirements.tex}
\label{apprequirement}

==> sections/usecase.tex <==
\subsection{Gesture Recognition to Control Appliances} 
\fakepar{Experimental Setup}
\begin{itemize}
    \item NLOS
    \item Light level?
\end{itemize}
\fakepar{Challenges}
\begin{itemize}
    \item Link obstruction when antenna is located close to the sensor
\end{itemize}

\fakepar{Solutions}
\begin{itemize}
    \item Moving the antenna away from the sensors
    \item Spreading
\end{itemize}



We investigate the feasibility of our system to detect hand gestures based on the key idea of VLS; a shadow cast over the light sensor such as a hand gesture will give rise to a unique pattern in the perceived light readings. Thus, when a particular hand gesture is performed over the light sensor, the gesture will manifest itself its output. We take advantage of this principle of to detect the presence of hand gestures using our passive switching sensors. We present four principal hand gestures that we can perform; swipe, taps, block, and swirl, as illustrated and explained in Figure~\ref{fig:gesture_one-sensor}. When one of these gestures are performed over a sensor, they are digitized by the 

%We present different hand gestures that we can perform based on the four principal hand gestures that we can perform; Swipe, Taps, Push, and Pull, as illustrated in Figure~\ref{fig:gesture_one-sensor}. These hand gestures can be used in combination to form more advanced gestures. For instance, a Push and Pull gesture can be combined to form a punch motion, or in reverse order to form a pump motion. When one of these gestures are performed over the visible light marker, they are digitized by the polymorphic digitization circuit and communicated via the SpreadScatter mechanism for the duration of the hand gesture event. 

Next, we use our combined sensor design consisting of four solar cells to detect directional information. The direction at which the hand is moving can be inferred by tracking the sequence of which sensors are obstructed at a particular time of an event. For instance, if sensors with ID 1 and 2, 3, and 4 are obstructed in order, then, it can be inferred that the hand is moving in a clockwise motion. Conversely, if sensors with ID 4, 3, 2, 1 are obstructed in order, the hand would be moving in a counter-clockwise motion. The sensor ID is determined at the receiver by observing the time difference between the end of the preamble and the beginning of the bit that indicates the activity of a particular solar cell. 

To be able to properly classify the hand gesture event, we make the assumption that we can sample RSSI fast enough at receivers to be able to accurately represent the timing of bit sequences transmitted by the SpreadScatter mechanism. Furthermore, we assume that we can collect RSSI samples for at least the full duration of the hand gesture event, which is defined by the time it takes for the SpreadScatter mechanism to transmit the entire frame, as shown in Figure~\ref{fig:packet}. Next, 
we evaluate hand gesture detection when backscattering signals at \SI{868}{\mega\hertz}, and we will use a multitude of CC1310 receivers to sample RSSI at different frequencies. We combine the signals from the receivers to reconstruct the transmitted stream of bits. 

We perform the experiment in an indoor office environment. We set up a \SI{868}{\mega\hertz} carrier source at approximately 1 meters away from the VLM and the CC1310 receiver approximately 4 meters away from the VLM and in non-line-of-sight. Next, we perform a hand gesture over the VLM and collect RSSI samples approximately every millisecond from the received backscattered signals.

%matching the first four bits which correspond to its preamble to a dictionary of preambles. 

%Since the length of the bit-sequence is known, the last bit marks 
%This is marked by the time after the last bit has passed, which can be determined by counting the transitions in RSSI values from the relative change in SNR. 

%We first identify the transmitting VLM lookup table to match its preamble to a identify the transmitting VLM by using a lookup table to match the preamble with the corresponding VLM.

%\subsubsection{Determining the Features and Generating Training Data}

\iffalse
\fakepar{Defining Gesture Features}
By collecting RSSI samples for the duration of a full hand gesture event, we can reconstruct the entire procedure at the receiver and perform classification to identify the event. For the classifier, we initiate a threshold which is equal to the digitized value corresponding to the mean ambient light level, and define three features based on it: gesture duration, drop duration, and rise duration. The gesture duration is defined as the time difference between the start and the end of a gesture, and is measured while the digitized values are below the threshold. The drop duration is defined as the time it takes for the received digitized values to fall from the threshold to the minimum, and rise duration is the reversed operation. 

Thus, we can generate training data for the classifier. To make the classifier agnostic to how different users perform the gestures shown in Figure~\ref{fig:gesture_one-sensor}, we construct the training data based on user input. The algorithm prompts a user to perform a particular gesture and labels the collected data accordingly. Next, the algorithm creates normal distribution around the collected samples to generate a larger and artificial training data set. Below is an example of how a user builds training data:

\fi

% Think about how 
%\begin{wrapfigure}{R}{0.5\textwidth}
%%%%
%        \begin{algorithm}[H]
%            \DontPrintSemicolon 
%            \SetAlgoLined
%            \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%            \Input{2D matrix consisting of \emph{binarySamples} and \emph{time}}
%            \Output{Training Data}
%            \BlankLine
%            risingEdges = time[binarySamples == 1]\;
%            fallingEdges = time[binarySamples == 0]\;
%            eventDuration = fallingEdges$_{i=1:end}$ - risingEdges$_{i=0:end}$\;
%            eventTimeDiff = risingEdges$_{i=1:end}$ - fallingEdges$_{i=1:end-1}$\;
            %labels$_i$ = 0 if eventDuration < userMaxSwipeDuration\;
            %labels$_i$ = 1 if eventTimeDiff < userMaxTapsDiff\;
%            %trainingData = Matrix(eventDuration, eventTimeDiff, labels)\;
%            \caption{Extracting 1-bit hand gesture information from a single sensor using matrix/vector operations.}
%        \end{algorithm} 
%%%
%\end{wrapfigure}

\iffalse
\fakepar{Implementation of Hand Gesture Classifier}
We use our polymorphic sensor to detect hand gestures at 1-bit and 4-bit, respectively, starting with a single light sensor. We implement a multiclass classification algorithm using a support vector machine (SVM). 
\fi

%\fakepar{Combining multiple light sensors to detect gestures}


%\begin{wrapfigure}{R}{0.5\textwidth}
%%%%%
    %    \begin{algorithm}[H]
    %        \DontPrintSemicolon 
    %        \SetAlgoLined
    %        \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
    %        \Input{Bit duration, time difference between events.}
    %        \Output{sensorID}
    %        \BlankLine
    %        sensorID = []\;
    %        \For{$i \in$ eventTimeDiff}{
    %            \uIf{i < bitDuration}{
    %                append(sensorID, 0)\;
    %            }
    %            \uElseIf{i < 2*bitDuration}{
    %                append(sensorID, 1)\;
    %            }
    %            \uElseIf{i < 3*bitDuration}{
    %                append(sensorID, 2)\;
    %            }
    %            \uElseIf{i < 4*bitDuration}{
    %                append(sensorID, 3)\;
    %            }
    %        }
    %        \Return sensorID
    %        \caption{Determining sensor Identifiers.}
    %        \end{algorithm} 
%%%%%
%\end{wrapfigure}

\fakepar{Experimental Evaluation}

\iffalse
\begin{itemize}
    \item Where to put this?
\end{itemize}
We perform the experiment in an indoor office environment. We set up a \SI{868}{\mega\hertz} carrier source at approximately X meters away from the VLM and the CC1310 receiver at X meters away from the VLM. Next, we perform a hand gesture over the VLM and collect RSSI samples approximately every millisecond from the received backscattered signals.
%\begin{wrapfigure}{R}{0.5\textwidth}
            \begin{algorithm}[h]
            \DontPrintSemicolon 
            \SetAlgoLined
            \KwResult{Write the result here}
            \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
            \Input{Training Data}
            \Output{Classifier}
            \BlankLine
             \eIf{condition}{
                instructions1\;
                instructions2\;
            }{
                instructions3\;
            }
            \caption{Hand Gesture Classifier}
        \end{algorithm}
%\end{wrapfigure}
\fi
%\begin{algorithm}
%\caption{Hand Gesture Classifier}
% \hspace*{\algorithmicindent} \textbf{Input} trainingData, labels \\
% %\hspace*{\algorithmicindent} \textbf{Output} leftPeak, rightPeak
%\begin{algorithmic}[1]
%\Procedure{Classifier}{}
%\State 
%\State svm\_model = SVM.fit(trainingData, labels)
%\end{algorithmic}
%\end{algorithm}

%\begin{itemize}
%    \item Classification accuracy (show confusion matrix)
%    \item Cross user accuracy
%\end{itemize}

\begin{figure}[!tb]
    \center
    \includegraphics[width=0.4\textwidth]{images/graphs/testplot.pdf} 
    \caption{\textit{Hand gesture classification accuracies.} }%
    \label{fig:hand-gesture-classification}%
\end{figure}
